Data-driven Design of Randomized Control Trials with Guaranteed Treatment Effects

Randomized controlled trials (RCTs) can be used to generate guarantees on treatment effects. However, RCTs often spend unnecessary resources exploring sub-optimal treatments, which can reduce the power of treatment guarantees. To address these concerns, we develop a two-stage RCT where, first on a data-driven screening stage, we prune low-impact treatments, while in the second stage, we develop high probability lower bounds on the treatment effect. Unlike existing adaptive RCT frameworks, our method is simple enough to be implemented in scenarios with limited adaptivity. We derive optimal designs for two-stage RCTs and demonstrate how we can implement such designs through sample splitting. Empirically, we demonstrate that two-stage designs improve upon single-stage approaches, especially in scenarios where domain knowledge is available in the form of a prior. Our work is thus, a simple, yet effective, method to estimate high probablility certificates for high performant treatment effects on a RCT.

==> meta.tex <==

\usepackage{aistats2025}
\usepackage{breakcites}
\usepackage{graphicx}
\newtheorem{assumption}{Assumption}
\usepackage{amsmath,amssymb,amsfonts,amsthm}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\usepackage{algorithm}
\usepackage{xcolor}
\usepackage{algpseudocode}
\usepackage{natbib}
\usepackage{bm}
\newcommand\E{\mathbb{E}}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\usepackage{bbm}
\usepackage{thm-restate}

% \theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{lemma2}[theorem]{Lemma} 

\newcommand{\Gap}[1]{\textcolor{red}{Gap: #1}}
\newcommand{\nrcomment}[1]{{\color{blue} Naveen: {#1}}}


==> old_writeup/old_writeup.tex <==


\section{Introduction}

% The "Contextual Bandits" problem has become a fruitful are of research on the last few years. The reason for this cornucopia of results (\Gap{ad citations})is that, the contextual bandits setting is generalization of the multi-armed bandit problem where the agent finding the best arm at a given time has access to relevant features ,a.k.a "Context", to make its decision.  \Gap{Should I talk about RL?}

% The mathematical formulation for the CB problem has been relatively stable: \Gap{Define it}. Usually, there are two learning tasks for the setting defined before: the policy optimization and the off-policy evaluation (OPE) [\cite{langford2007epoch} \cite{dudik2011doubly}, \cite{li2010contextual}]. 

% Being the OPE a counterfactual problem, it raises the question if it can be written using the potential outcomes language. Indeed, there is a close relationship between the OPE and the so called \textit{stochastic interventions} in causal inference; we recommend the reader the discussion about this topic done by \cite{waudby2022anytime} in the appendix of the cited article. Traditionally, the CB problem has not be written using this language (\Gap{add  citations}). However, recently the OPE problem framed as a potential outcomes problem has received a lot of attention because it allows to perform online interventions while allowing to perform inference on several statistics [\cite{bibaut2021post}, \cite{zhang2021statistical} \cite{zhan2021off}] product of running a policy search in an online fashion.

% The reason behind this recent push for developing causal inference on top of online interventions is because they open the door to adaptive experimental designs. These experiments allow to improve efficiency on particular tasks [\Gap{citations}] while deployed in an online-fashion, i.e, on a continuous stream of not necessarily i.i.d data, making the experimental framework overall way more flexible than for example traditional randomized control trials. \Gap{Rephrase (copy paste)} However,  once  the  experiment  is  over,  we  are  often  interested  in  using  the  adaptively  collected  data  to  answer  a  variety  of  questions,  not  all  of  them  necessarily  targeted  by  the design. For example, a company experimenting with many types of  web  ads  may  use  a  bandit  algorithm  to  maximize  click-through  rates  during  an  experiment,  but  still  want  to  quantify the  effectiveness  of  each  ad.  At  this  stage,  fundamental  tensions  between  the  experiment  objective  and  statistical  inference become apparent: Extreme under sampling or nonconvergence  of  the assignment  probabilities  make  reusing  these data challenging \cite{athey2022contextual}.

% There has been very few results exploring this trade-off between policy learning for maximizing the welfare during an interventions versus policy learning for maximizing welfare after the intervention [\cite{athey2022contextual} \cite{li2010contextual} \cite{bastani2021efficient} \cite{kasy2021adaptive}, \cite{deshmukh2018simple}, \cite{chambaz2017targeted}]. We are interested in exploring these interplay and gain some more intuition on how antipodal these two objectives are. \Gap{Why is this literature small and niche? what problems do they solve? why they say the lit is not thoroughly explained?}.  In particular, \cite{athey2022contextual} claims that there is no results about limitations of algorithms for policy learning (simple regret minimization). Their claim is that there is no work exploring the range of models or conditions under which that were explicitly designed for policy learning end up performing worse than an uniform sampling baseline (RCT). However, the authors cite the work of \cite{bubeck2011pure} which provides, for the case of a finite number of arms, a lower bound on the simple regret that depends on the cumulative one: the smaller the latter, the larger the former. A result that is consistent with the uniform sampling being a strong baseline.


% The practical limitations of algorithms designed for policy learning have not been fully explored in the literature. In particular, we are not aware of research documenting findings analogous to our result that in a range of outcome models consistent with our pilot data, uniform (nonadap- tive) sampling performs better than algorithms that were explicitly designed for policy learning, though the fact that uniform sampling is in general a strong baseline is suggested by the theoret- ical results in Bubeck et al. (2009). The findings in this paper suggest that there is still room for improvement in algorithms designed for policy learning, and also for algorithms that optimize for regret in a contextual bandit settings; see Krishnamurthy et al. (2021); Krishnamurthy and Athey (2021); Carranza et al. (2022); Simchi-Levi and Xu (2022) for some recent discussions of challenges for standard algorithms that arise when the functional form of the mapping between individual characteristics and outcomes is unknown.



% Such way of conducting experiments can dramatically improve efficiency for particular objectives: maximizing welfare during the  experiment  (1,  2)  or  after  it  (3,  4);  quickly  identifying  the best treatment arm (5, 6); maximizing the power of a particular hypothesis (7–9); and so on. To achieve these efficiency gains,we adaptively choose assignments to resolve uncertainty about some aspects of the data-generating process, at the expense of learning  little  about  others.  For  example,  welfare-maximizing designs tend to focus on differentiating optimal and near-optimal treatments,  collecting  relatively  little  data  about  suboptimal ones.


%  The first goal is to use the data from the experiment to design an effective targeted treatment assignment rule at the end of the experiment. Our second goal is to avoid assigning observations to subopti- mal treatment arms during the experiment, and in particular, to target treatment assignments to individuals on the basis of their observed characteristics (their “contexts”).

%   the trade-off between the goal of maximizing outcomes for the participants in the experiment and our first goal of policy learning.

%   Our paper is one of a small number (e.g., Li et al. (2010) and Bastani et al. (2021)) that has conducted a contextual bandit in practice and analyzed its performance relative to alternatives

%   However, it turns out that the two goals are partially in conflict. As we demonstrate using simula- tions designed based on our pilot data, the true value of the best policies estimated from adaptive data collection is often lower than that of the best policies estimated from nonadaptive data col- lection, such as through a randomized control trial with uniform assignment probabilities.

%   Our main experiment has two phases: the learning phase and the evaluation phase. The goal of the learning phase is to learn a treatment assignment policy, balancing exploration and exploitation with both cumulative regret and policy learning. 

% In terms of obtaining high rewards during the experiment (i.e., cumulative regret minimization), the bagging algorithm described above often performs similarly to other optimal bandit algorithms (Bietti et al., 2018). However, as we demonstrate in the next section, when we use data collected via this heuristic to learn a policy (i.e., simple regret minimization), we often end up with a policy whose value is relatively low (i.e., the approach is not successful at identifying the best policy assignment rule, which is one of our stated goals). In fact, we are often better off collecting data by assigning arms uniformly at random.

% , there is no general-purpose computationally efficient algorithm for pure exploration objectives like simple regret minimization in the contextual bandit setting. Further, there has been relatively little work so far into algorithms that explore the trade-off between multiple objectives like cumulative regret and simple regret

% RCTs are expensive and require a significant amount of resources to set-up. Usually the deliverable after performing an RCT is an estimate of the ATE on top of which statistical inference can be performed. More formally, at the end of an RCT there should be statistical evidence of the realized intervention impact. However, in high-stakes settings in which the data may be scarce, the cost of a wrong decision is very high. Thus, we aim to correctly identify at least a single good intervention.
% Our proposal is to deliver a certificate for an intervention, meaning we will provide statistical evidence that at least one of the interventions is guaranteed to have a positive impact. To achieve this, we propose a warm-up stage to discard ineffective arms, thereby maximizing the power of our certificate in the second stage.


RCTs are expensive and require a significant time and work to set-up. Usually the deliverable after performing an RCT is an estimate of the ATE on top of which statistical inference can be performed. More formally, at the end of an RCT there should be statistical evidence of the realized intervention impact. However, in high-stakes settings in which the data may be scarce, the cost of a wrong decision might be very high. Thus, we aim to guarantee to identify at least a single high-impact intervention. 

For us, impact is going to be a synonym of \textit{certification}, in plain English, we are interested in estimating the lowest possible ATE of a particular treatment assignment on an RCT with high probability. Our proposal is to derive such \textit{certification} by the means of a two satge approach. The idea is to be able to discard interventions with a possibility of a very low impact on the first stage (i.e being able to discard ineffective arms), thereby maximizing the power of our certificate in the second stage.
 
%To drive product innovation and augment man- agerial decision-making, it is often necessary to understand how much an additive feature moved some user metric, not just whether it did or not

%As drugs often come with side effects or have interactions with other medications, having statistical inference on the treatment effect be- tween the various drugs and/or doses being compared is important to guide policies around which drug and/or dose should be prescribed given different patient histories 


%While Inverse Propensity Weighting (IPW) estimators are often unbiased in the MAB setting (Horvitz and Thompson 1952; Hadad et al. 2021), their variance can explode, thus making any subsequent hypothesis testing on the ATE essentially powerless.

\subsection{Problem formulation}
Now that the problem is motivated, the formal concepts necessary for a thorough analysis will be introduced. Lets begin with the definition of a certificate.

\begin{definition}
Let $(l,h)$ be an interval such that $\mu$ belongs to it with probability $1 - \delta$. We will say that $l$ is a certificate for $\mu$.
\end{definition}

Let $\mathcal{A}$ the set of all arms. Thus, to analyze  the performance of any algorithm that outputs a certificate, we are interested in producing a lower bound for
\begin{align*}
    \E[\max_{i \in B}\l_i]
\end{align*}

Note how the expectation is on both the choosing of the set $B$ and the observed $l_i$ on the second stage. Of course this lower bound is a function on the policy used to choose the set $B$. 


\subsection{Power analysis}

\Gap{Small analysis to talk about how the power improves as a consequence of the two staged approach}

\subsection{Related work}

% Adaptive experimental design, 


\textbf{Learning efficiency} \cite{fan2021fragility}, policies under very general assumptions achived from optimal cumulative regret optimization algorithms end up having heavy tails distributions.


\textbf{Adaptive experimental design}
\cite{simchi2023multi} Offers an interesting formalization of the trade off between minimizing regret (maximizing welfare during an intervention) and mean squared estimation n error. The authors deal with these trade off by framing and minimax optimization problem where Pareto improvements are achieved for both the regret and the estimates of the ATE. Then proposes a variation of the EXP3 algorithm (cite). 

\textbf{Inference}
\cite{liang2023experimental} Uses a mixture model between a bandit algorithm and a Bernoulli trial at time $t$ . This way is able to provide any time valid confidence sequences to allow for inference on the ATE with high statistical power. They provide an asymptotic confidence sequence \cite{waudby2021time} for their ATE estimator.

\cite{hadad2021confidence} Not as relevant, they have a very good introduction, the result is another asymptotically normal ATE estimator.

\cite{chen2023optimal} Is interested in last batch-only inference, that is, inference if data is conditioned on fixed $(T, \pi_{1:T}, \eta)$, This translates is once the experiment is stopped it can be restarted. $\eta$ is weights for every mean of the reward of each arm, this might come in handy if I desire to add more weight to a particular reward with higher expected reward.  then any confidence set which is valid conditional on $(T, \pi_{1:T}, \eta)$ must also be valid conditional on $x_1 : T - 1$. In fact, simply requiring conditional coverage given $\eta$ is already sufficient to obtain this conclusion. This effectively means we cannot use information from the first $T - 1$ batches of data, so it is impossible to improve on the power of last-batch-only inference without losing some degree of robustness.

% \textbf{look for:}
% Non contextual setting, look for literature. Adaptive clinical trial, two stage experimental design, Adaptive experiments. 

\section{Two staged RCT}

Let $Z_1,...,Z_N$ be the whole sample. Let $X_1,...,X_n$ the data set aside for the first stage and $Y_1,...,Y_m$ the data set aside for the second stage. It follows that $n + m = N$. Furthermore, let all the arms be distributed as Bernoulli random variables. Lets suppose that there are $K$ such treatments as well. From now on, to this vector of treatments we will refer as $\mu$. We are assuming an uniform allocation strategy for all arms at any give stage of the trial.

\begin{definition}
    A certificate $l_i$ for $\mu_i$, is a random variable such that $l_i < \mu_i$ with probability at least $1 -\delta$
\end{definition}


% \Gap{Explain the algorithm and how  it differs from best arm, top-k and $\epsilon$ best arms}

% \Gap{Veryfing and arm and finding it have different complexities.}

We are interested in finding the highest of such possible certificates among the arms $\mu$. To that effect, we propose a two stage approach. In the first stage, we are interested in obtaining a set $B$ from a policy $\pi$, while at the second stage we are interested in finding $l$, the best certificate in $B(X)$. It is worth noticing, that the randomness behind a particular chose of the set $B$ is driven only by the data from the first stage, $X_i$, while the randomness from the bound $l_i$, arises from the second stage sample. 


Let $\pi(X)$ denote a policy that maps from a realized first-stage sample $X$ to a set of arms. Given a fixed set of arm means $\mu_1...\mu_K$, we define the expected value of a fixed $\pi$ to be
\begin{align*}
    f_\mu(\pi) = \E_{X \sim \mu}\left[\max_{i \in \pi(X)}l_i\right]
    \label{objective}
\end{align*}
% We are interested in policies that compete with the optimal value:
% \begin{align*}
%     OPT(\mu) = \max_\pi f_\mu(\pi).
% \end{align*}

% Formally, we are interested in optimizing the objective, 
% \begin{align}
%     f (\pi) = \E\left[\max_{i \in \pi(X)}\mu_i - \sqrt{\frac{2}{|m|}log(\frac{2}{\delta})}\right]
%     \label{objective}
% \end{align} 
% where the expectation is taken both over $X$ and $Y$.


\textbf{Second stage.} Towards the aim of analyzing the objective \ref{objective}, lets start by analyzing the second stage. Naturally, lets condition on a draw from the first stage. Therefore, we are fixing a particular output of a fixed policy $\pi$: a set $B$ of size $k$. By Hoeffding's inequality:

\begin{align*}
    P\left(|\overline{Y}_i - \mu_i| < \sqrt{\frac{2}{|m/k|}log(\frac{2}{\delta})}\right) \geq 1 - \delta
\end{align*}

Therefore $\overline{Y}_i -\sqrt{\frac{2}{|m/k|}log(\frac{2}{\delta})}$ is a certificate of $\mu_i$. Throughout on we will denote $\sqrt{\frac{2}{|m/k|}log(\frac{2}{\delta})} = c(k)$.

\textbf{First stage.} Analyzing the first stage is more complicated as the expectation in \ref{objective} varies over all possible sets $\pi(x)$. Lets start analyzing a simple policy $\pi$, $\pi(X) = \{ \argmax_{i} \overline{X}_i = j \}$ (i.e $|\pi(X)|=1$). The final objective in this case becomes:
\begin{align*}
    f(\pi) = \E\left[\overline{Y}_j - \sqrt{\frac{2}{|m|}log(\frac{2}{\delta})}\right]
\end{align*}
Note how there is randomness in $\overline{Y}$ and in $j$.  Now, we proceed to analyze the expected value of the error of our two stage certificate. Let $\mu_{i^*}$ be the expected value 
of the treatment with the highest reward, then
\begin{align}
    \E[\mu_{i^*} - (\overline{Y}_j - \sqrt{\frac{2}{|m|}log(\frac{2}{\delta})}] = \E[\mu_{i^*} - \mu_j ] + \sqrt{\frac{2}{|m|}log(\frac{2}{\delta})}
\end{align}
Where the final expectation is taken over $X$. Then using the bounds derived from  \cite{bubeck2011pure} we can produce the following bound:
\begin{align}
    \E[\mu_{i^*} - (\overline{Y}_j - \sqrt{\frac{2}{|m|}log(\frac{2}{\delta})}] \leq \\
    \sum_{i=1}^K \Delta_i exp(-\Delta_i \frac{n}{K}) + \sqrt{\frac{2}{|m|}log(\frac{2}{\delta})}
\end{align}
Note how this bound is concordant wth the intuition: a bigger $n$ decreases the first term on the bound but increases the second (as $n+m = N$) and vice versa.

\begin{itemize}
    \item Note how the first term decreases way faster than the second one ($\frac{1}{e^n}$ vs, $\sqrt{m}$).
    \item This bound has the nice property that the first part also controls for small values of $\Delta$. The regret is small in such case even though the probability of making a mistake is not small. This can be seen in the $\Delta$ term  accompanying the $exp$ term. 
\end{itemize}

\section{Top-K policy reduction}

How can we extend our previous simple analysis to a general policy $\pi$?. Lets begin by assuming $|B|>1$ otherwise it will be the special case analyzed in the last section. As a consequence of the uniform allocation and that $|B| = k > 1$, then the initial Sub-Gaussian bound is transformed to $$\mu_i > \overline{Y}_i -\sqrt{\frac{2}{|m/k|}log(\frac{2}{\delta})}$$ with probability at least $1 - \alpha$. 

Let $\sigma(X)$ be a permutation of the arm indices in order of empirical mean in the sample $X$. If there are ties in the empirical means, they are broken by drawing uniformly distributed random variables $r_i$ for each arm. A top-k policy outputs sets of the form
\begin{align*}
    \pi(X) = \{\sigma(X)_1, \sigma(X)_2...\sigma(X)_k\}
\end{align*}
for some function $k(X)$ (i.e., the number of arms chosen may depend on the sample). For convenience, define $B(X)_k$ to be the top-k set above. 



\textbf{Assumption:} There is an ordering of the arms by first-order stochastic dominance. i.e., $X_1$ stochastically dominates $X_2$ and so on. This holds if the arms have binary outcomes. This assumption is useful  because first claim that the value $OPT(\mu)$ must be achieved by a policy that takes a ``top-k" form.
% For continuous outcomes, it may require some sort of homoskedasticity (e.g., if the rewards are Gaussian it may require the variances to be equal). 

    
In other words, if the arms are stochastically dominated, it is enough to analyze the subset of top-k policies. Such analysis starts with a technical lemma. First, we will analyze the case where the two policies differ only on the last element chosen. That is, 
\begin{align*}
    &\pi(X) = \{\sigma_1(X), \sigma_2(X), ..., \sigma_{k(X) - 1}(X), \sigma_j(X)\}, j > k \\
    &\pi'(X) = \{\sigma_1(X), \sigma_2(X), ..., \sigma_{k(X) }(X)\}
\end{align*}


% Sub-lemma: for any $i < j$, $\mu_{\sigma_i(X)}$ first-order stochastically dominates $\mu_{\sigma_j(X)}$. (This makes the proof much easier but I'm not sure if it's true for arbitrary distributions. It should be true if, e.g., the outcomes are all binary variables with different success probabilities).
	\begin{lemma}
		For any $i < j$, $\mu_{\sigma_i(X)}$ first-order stochastically dominates , $\mu_{\sigma_j(X)}$ 
	\end{lemma}
	\begin{proof}
		Fix a given $t$. We compare $\Pr(\mu_{\sigma_i(X)} \geq t)$ and $\Pr(\mu_{\sigma_j(X)} \geq t)$ via  a coupling argument where we fix the mean of every position in the permutation except for positions $i$ and $j$. Formally, we decompose
		\begin{align*}
			\Pr(\mu_{\sigma_i(X)} \geq t) - \Pr(\mu_{\sigma_j(X)} \geq t) =\\ \E[1[\mu_{\sigma_i(X)} \geq t] - 1[\mu_{\sigma_j(X)} \geq t]]\\
			= \E[\E[1[\mu_{\sigma_i(X)} \geq t] - 1[\mu_{\sigma_j(X)} \geq t]|\mu_{\sigma_k(X)}, k \neq i,j]].
		\end{align*}
		We will show that the inner expectation $\E[1[\mu_{\sigma_i(X)} \geq t] - 1[\mu_{\sigma_j(X)} \geq t]|\mu_{\sigma_k(X)}, k \neq i,j]$ is always nonnegative. After conditioning on $\mu_{\sigma_k(X)}, k \neq i,j$, there are two possible values for $\mu_{\sigma_i(X)}$ and $\mu_{\sigma_j(X)}$ (i.e., the means of the two arms that did not appear in other positions of the permutation). Denote these values by $\mu_a$ and $\mu_b$ where $\mu_a \geq \mu_b$ refers to the larger of the two. There are two cases. The first case is where either $\mu_a \geq \mu_b \geq t$ or $t \geq \mu_a \geq \mu_b$. Denote this event as $\mathcal{E}_1$. By definition,   $\E[1[\mu_{\sigma_i(X)} \geq t] - 1[\mu_{\sigma_j(X)} \geq t]|\mathcal{E}_1, \mu_{\sigma_k(X)}, k \neq i,j] = 0$. The second case is that $\mu_a \geq t > \mu_b$. Denote this event as $\mathcal{E}_2$. Since $i < j$, $\sigma_i(X) = a$ if and only if $\overline{X}_a > \overline{X}_b$, which in turn implies that  $\mu_{\sigma_i(X)} \geq t$ if and only if either $\overline{X}_a > \overline{X}_b$ or  $\overline{X}_a = \overline{X}_b$ and $r_a > r_b$.  Because $\mu_a \geq \mu_b$, the assumption of a stochastic dominance ordering on the arms combined with independence of the samples implies that  $Pr(\overline{X}_a > \overline{X}_b|\mathcal{E}_2, \mu_{\sigma_k(X)}, k \neq i,j) \geq Pr(\overline{X}_b > \overline{X}_a|\mathcal{E}_2, \mu_{\sigma_k(X)}, k \neq i,j) $. Moreoever, whenever $\overline{X}_a = \overline{X}_b$, $\Pr(r_a > r_b) = \frac{1}{2}$ by definition.  Since conditioned on $\mathcal{E}_2$, $1[\mu_{\sigma_j(X)} \geq t] = 0$ whenever $1[\mu_{\sigma_i(X)} \geq t] = 1$, we conclude that $\E[1[\mu_{\sigma_i(X)} \geq t] - 1[\mu_{\sigma_j(X)} \geq t]|\mathcal{E}_2, \mu_{\sigma_k(X)}, k \neq i,j] =\geq 0$ and the lemma follows.
	\end{proof}

\begin{lemma}
    Fix an arbitrary policy $\pi$. Define its top-k counterpart $\pi'$ to be the top-k policy with $k(X) = |\pi(X)|$. That is, it selects the same number of arms as $\pi$ does for every realization of the sample, but it selects those arms to be the ones with largest empirical mean, then $f(\pi') \geq f(\pi)$.    
\end{lemma}
\begin{proof}
    We conclude that since $\max_{i \in \pi(X)}\{\mu_i\}$ is a non-decreasing function in arguments $\{\mu_i: i \in \pi(X)\}$, first-order stochastic dominance implies (Is equivalent to the expectations matching for every non decreasing function).
\begin{align*}
    \E[\max_{i \in \pi'(X)}\mu_i] \geq \E[\max_{i \in \pi(X)}\mu_i]
\end{align*}
from which it follows that $f(\pi') \geq f(\pi)$     
\end{proof}



% Next step: use this to chain together an argument for the general case, by considering a sequence of intermediate policies that change one arm at a time. 


% Let $m(X) = \arg\max_{i \in \pi(X)} \mu_i$ and $m'(X) = \arg\max_{i \in \pi'(X)}$ be the arm achieving the max value of $\mu$ for the two algorithms. One of four events must always hold, and we will decompose the expected reward according to these cases:
% \begin{align*}
%     \mathcal{E}_1: m(X) \in \{\sigma_1(X), \sigma_2(X), ..., \sigma_{k(X) - 1}(X)\}, m'(X) \in \{\sigma_1(X), \sigma_2(X), ..., \sigma_{k(X) - 1}(X)\}\\
%         \mathcal{E}_2: m(X) \in \{\sigma_1(X), \sigma_2(X), ..., \sigma_{k(X) - 1}(X)\}, m'(X) \in \{\sigma_1(X), \sigma_2(X), ..., \sigma_{k(X) - 1}(X)\}

% \end{align*}



% The first case is where these arms are the same (i.e., correspond to one of the first $k(X) - 1$ arms). If this case does not obtain, we must have that $m'(X) = \sigma$
% \begin{align*}
%     &\E[LB(\pi'(X)) - LB(\pi(X))]\\ &= \E[\mu_{m'(X)} - \mu_{m(X)}]\\
%     &= \Pr[m(X) = m'(X)]\E[\mu_{m'(X)} - \mu_{m(X)}| m(X) = m'(X)] + \\
%     &\Pr[m(X) \in \{\sigma_1(X)...\sigma_{k(X) - 1}(X)\}, m'(X) = \sigma_{k(X)}(X)]\E[\mu_{m'(X)} - \mu_{m(X)}| m(X) \in \{\sigma_1(X)...\sigma_{k(X) - 1}(X)\}, m'(X) = \sigma_{k(X)}(X)]\\
%     &+ \Pr[m(X) \in  \{\sigma_{k(X) + 1}(X)...\sigma_{K}(X)\}, m'(X) = \sigma_{k(X)}(X)]\E[\mu_{m'(X)} - \mu_{m(X)}| m(X) \in \{\sigma_{k(X) + 1}(X)...\sigma_{K}(X)\}, m'(X) = \sigma_{k(X)}(X)]
% \end{align*}
% Clearly for the first term, we have $\E[\mu_{m'(X)} - \mu_{m(X)}| m(X) = m'(X)] = 0$. 


\begin{theorem}
    For any $\mu$, there exists a top-k policy $\pi$ such that $OPT(\mu) = f(\pi)$. Pick the optimal policy $\pi^*$, i.e $arg\max_{\pi} f_{\mu}(\pi) = \pi^*$ then $\pi^{*'}$ (its corresponding top-k policy) is also optimal.
\end{theorem} 
% Let define the \textit{observed expected value} of a policy $\pi$ as $$g(\pi) = \E[\max_{i \in \pi}\overline{Y}_i - c(|\pi(X)|)]$$

% Using the same naming conventions as for $f$, let $\pi$ be a policy and $\pi'$ is top-k counterpart.

% \textbf{Claim} $|g(\pi) - g(\pi')| \leq \epsilon$ or maybe $g(\pi'k) \leq g(\pi)$

% Lets denote $\pi^*$ the optimal top-$K$ policy for $f$ and $\pi"$ the optimal $K$ policy for $g$. If the claim is true, there is a clear strategy to follow:
% \begin{itemize}
%     \item The optimal $f(\pi_f)$ is bounded by the top-k $f(\pi^*)$.  
%     \item The optimal $g(\pi_g)$ is bounded by the top-k $g(\pi")$.  
%     \item $g(\pi")$ is close to $f(\pi^*)$
%     \item we can bound  $g(\pi)$ by bounding $f(\pi^*)$.
% \end{itemize}

% That is to reduce the problem of finding a lower bound on the \textit{observed expected value} on all the policies $\pi$ to instead find a bound on the expected values of top-k policies. 

% We would like to control for 
% $$|g(\pi") - f(pi^*)|$$

% It must be true that,
% \begin{align*}
%     \E[\max_{i \in  \pi"}\overline{Y}_i - c(|\pi"(X)|)] -\E[\max_{i \in  \pi^*}\mu_i - c(|\pi"(X)|)]\\
%     \E[\max_{i \in  \pi"}\overline{Y}_i - \max_{i \in  \pi^*}\mu_i] - \E[c(\frac{k' - k}{m})]
% \end{align*}
% This formulation is nice because the first term will be controlled by $n$ and the second by $m$. Naturally as $n + m$ is a fixed quantity, both terms can not be controlled for at the same time. 

% \cite{athey2022contextual}

As a consequence of theorem 1 it suffices to compete with the best top-k policy in order to compete with $OPT(\mu)$. However, non of this results say anything about the optimal $k$; it remains a problem how to pick the adequate $k$.

\textbf{Algorithm} We proposed the algorithm \ref{algo_1} based on sample splitting to pick the $k$.
\begin{algorithm}
\caption{Sample splitting algorithm}
\begin{algorithmic}[1]
\State \textbf{Input:} $T$ iid samples.
\State \textbf{Output:} certificate $l_i$ and set $\pi(X)$
\State Split first stage data randomly into two sets. $ train = \{x_1,...,x_{\frac{n}{2}}\}$ and $val=\{z_1,...,z_{\frac{n}{2}}\}$.
\State compute $\{\overline{x}_1,...,\overline{x}_K\}$ and $\{\overline{z}_1,...,\overline{z}_K\}$.
\State Sort $train$ and let $\sigma$ be the permutation that leads to the ordering of the resulting indexes.
\State Apply $\sigma$ to $test$ 
\For{$i = 1$ to K} 
    \State set $aux_i = \argmax test[1:i] + \sqrt{\frac{2}{|m/i|}log(\frac{2}{\delta})}$
\EndFor
\State $k = \argmax aux_i$
\State \Return $aux_i$, $k$
\end{algorithmic}
\label{algo_1}
\end{algorithm}

Define the number of arms selected by the optimal k-policy $\pi^*$ as $k_*(X)$. trough out, we will refer to the number $k^*$ as omniscient. We now show that the reward of the $k$ picked by this algorithm is bounded below. The xact bound is exposed in the follwoing theorem


% Claim: let $\pi_*$ be a top-k policy achieving value $OPT(\mu)$ and $\pi_{omni}$ be the top-k policy that selects $k_{omni}(X)$ arms. Then, $f(\pi_{omni}) \geq f(\pi_*) = OPT(\mu)$. 

% Next, we introduce an easier-to-analyze version of sample splitting algorithm. This algorithm gets to see both the original sample $X$ as well as another sample $Z$ of equal size, distributed the same as $X$ (i.e., sampled iid according to $\mu$). We will prove that the sample splitting algorithm competes with $\pi_{omni}$. The catch is that it gets to use twice as much data. Later, we will prove that if it uses the real number of samples, its regret compared to $OPT(\mu)$ grows by only a bounded amount. 

% The sample splitting algorithm estimates the mean of each arm on $Z$ as $\hat{\mu}_i(Z)$. Then, it estimates the objective function as 
% \begin{align*}
%     \widehat{LB}(B(X)_k) = \max_{i=1...k} \hat{\mu}_i(Z) - c(k).
% \end{align*}
% Finally, it selects the top $\hat{k}(X) = \arg\max \widehat{LB}(B(X)_k)$ arms. Denote this policy as $\pi_{split}$. Suppose that for all $k$, we have that 
% \begin{align*}
%     | \widehat{LB}(B(X)_k) -  LB(B(X)_k)| \leq \epsilon
% \end{align*}
% for some $\epsilon > 0$.  We must have that 
% \begin{align*}
%     LB(B(X)_{\hat{k}}) \geq \max_\ell LB(B(X)_\ell) - 2\epsilon
% \end{align*}
% \Gap{This must be proven, in principle $\hat{k}(X) \neq k(X)_{omni}$}

% and so taking expectations over $X$ yields that 
% \begin{align*}
%     f(\pi_{split}) \geq f(\pi_{omni}) - 2\epsilon \geq OPT(\mu) - 2\epsilon.
% \end{align*}
% Now, $\pi_{split}$ is not actually implementable because we do not get to see an extra sample $Z$; rather, we must split the original sample $X$ in some manner. This can be phrased as that we compete with $\pi_{omni}$ for an instance with $\frac{n}{2}$ samples, and now we need to relate this to the corresponding $\pi_{omni}$ with $n$ samples. 




\begin{proposition}
Let $\mu$ be any distribution of arms, let $\{\sigma_1(X),...,\sigma_K(X)\}$ a permutation of the indexes of arms ordered by sorting the empirical means observed on the first stage. Then for any top-i policy $\pi^i$, the expected value of its certificate $f(\pi^i)$  is bounded below by 
\begin{align*}
    f(\pi^*)\\  
    - \sum_{j = 1}^* exp(\frac{-2[\Delta_{*i}- (c(*) - c(i)) ]^2n}{2K})[\Delta_{*i} - (c(*) - c(i))] \\
    - \sum_{j = *+1}^K exp(\frac{-2\Delta_{i*}^2n}{2K})[\Delta_{*i} - (c(*) - c(i))]
\end{align*}

\end{proposition}
\begin{proof}
    Let,

\begin{align*}
    &\pi(X) = \{\sigma_1(X), \sigma_2(X), ..., \sigma_{k(X) - 1}(X), \sigma_j(X)\}
\end{align*}
 the permutations that orders the empirical means from the first stage from lowest to highest.

  As a consequence of the stochastic dominance it suffices to focus on top-k policies. Let $\pi^*$ be the optimal top-$k$ policy. Let $\pi^i$ be a top $i$ policy where $k\neq i$. Clearly
 \begin{align*}
     f(\pi^*) - f(\pi^i) =  \E[\max_{i \in \pi^*(X)}\mu_i - c(*)] - \E[\max_{j \in \pi^i(X)}\mu_i - c(i)]
 \end{align*}

The sample splitting algorithm:
\begin{itemize}
    \item First use one of the samples to estimate the order of the $\mu_{\sigma_i(x)}$.
    \item Pick $i$, such that $\overline{Z}_i - c(i)$ is the largest. Note that indexes are given by the first stage data.
\end{itemize}


 
 \textbf{Case 1}, $i < *$. In this scenario, $c(*) - c(i) \geq 0$ hence if $\max_{ j \in \pi^i(X)}\mu_j \geq \max_{ j \in \pi^*(X)}\mu_j$ that will contradict the optimallity of $\pi^*$, furthermore, this is true for every $i < *$, thus concluding that $\mu_{\sigma_*(X)} > \mu_{\sigma_i(X)}$ (not even $\geq$ ).  Adittionally by optimality of $*$, $\mu_* - c(*) > \mu_i - c(i)$, if $\overline{Z}_i - c(i)> \overline{Z}_* - c(*)$ then given that $c(*) - c(i) < \mu_* - \mu_i$. In particular:
 \begin{align*}
    &\leq \sum_{j = 1}^* P(\overline{Z}_* - \overline{Z}_i -c(*) +c(i) < 0)[\Delta_{*i} - (c(*) - c(i))]\\
    &\leq \sum_{j = 1}^* exp(\frac{-2[\Delta_{*i}- (c(*) - c(i)) ]^2n}{2K})[\Delta_{*i} - (c(*) - c(i))]
 \end{align*}

 

 \textbf{Case 2} $* < i$, $c(*) - c(i) < 0$, thus as $\overline{Z}_* - \overline{Z}_i < c(*) - c(i)$ (Otherwise the index $i$ would not have been picked) then it must be concluded that $\overline{Z}_* - \overline{Z}_i < 0$. Then we can bound this terms using the event $P(\overline{Z}_* - \overline{Z}_i < 0)$ in which the traditional Hoeffding's bound trick can be plugged.

\begin{align*}
    &\leq \sum_{j = *+1}^K P(\overline{Z}_* - \overline{Z}_i < 0)[\Delta_{*i} - (c(*) - c(i))]\\
    &\leq \sum_{j = *+1}^K P(\overline{Z}_* - \overline{Z}_i - \Delta_{*i}< -\Delta_{*i})[\Delta_{*i} - (c(*) - c(i))]\\
    &\leq \sum_{j = *+1}^K exp(\frac{-2\Delta_{i*}^2n}{2K})[\Delta_{*i} - (c(*) - c(i))]
\end{align*}
Note that although $\Delta_{*i}$ might be negative, $\Delta_{*i} - (c(*) - c(i))$ is not by optimality of $*$. Conditional on $X$



 The inequality comes as a consequence that if there is any regret is because the wrong arm was picked, thus the certificate was better.
\end{proof}





 \Gap{There is not optimal n or m}



\section{Extensions}

This work so far has been focused on bounding all possible choices of $\mu$. In particular, our bound  can be seen as an estimation of a min-max guarantee:
\begin{align*}
    \min_{\mu} \max_{\pi} f_\mu(\pi)
\end{align*}

Hence, without prior knowledge on the distribution, a bound dependant on the data is provided, thus guarantying a valid bound for all distributions $\mu$.

However, lets suppose for a moment that there is a prior on the distribution $\mu$. In this scenario our problem of interest gets reduced to:
\begin{align*}
    \min_{\rho \in U}\max_{\pi}f_{\mu}(\pi)
\end{align*}
Where $U$ bakes the prior knowledge on the distribution, reducing the problem to a subset of of distributions we are interested in. This presentation is usually refered in the literature as \textit{distributionally robust optimization}.

One special case of the previous setting is the so called \textit{stochastic regression} problem. On it, the distribution is fully known, thus reducing the problem to an stochastic optimization one.
\begin{align*}
    \max_{\pi}f_{\mu}(\pi)
\end{align*}

The dependency on $\mu$ can also be seen as a feature of this setting as it allows to encode prior information that might be available from the distribution. Such domain knowledge can be encoded in our problem as a Bayesian prior, thus making $\mu$ a random variable and transforming our objective into:

\begin{align*}
    \argmax_{\pi} \E_{\mu \sim P}[\E_{X \sim \mu}[f_{\mu}(\pi(X))]]
\end{align*}

 However, recall the fact that $f_{\mu}(\pi(X)) = \max_{\i \in B(X)} \mu_i - O(\sqrt{\frac{|B|}{m}})$, which leads to the question we faced in the min-max setting analyzed before; how can we approximate $ \max_{\i \in B(X)} \mu_i$? 

A possible solution will be to run a greedy search to craft the set $B$, as $\max$ is a submodular function. Then, the algorithm will compute via Montecarlo approximation a estimate of $E_{\mu \sim p(\mu|x)}[f_{\mu}(\pi(X))]$ and then greedily update the set $B$, thus creating an estimate for:
\begin{align*}
    \max_{|B| \leq k} \E_{\mu \sim p(\mu|x)}[f_{\mu}(\pi(X))]
\end{align*}

Which naturally will gave us an estimate of 
\begin{align*}
    \argmax_{\pi} \E_{\mu \sim p(\mu|x)}[f_{\mu}(\pi)]
\end{align*}

Note that 
\begin{align*}
    \E_{\mu \sim P}[\E_{X \sim \mu}[f_{\mu}(\pi(X))]] = \E_{X \sim \mu}[\E_{\mu \sim p(\mu|X)}[f_{\mu}(\pi(X))|X]] 
\end{align*}
Hence as $\pi$ is a function of $X$ the solution to the posterior will be the optimal.

\subsection{Upper bound on submodular estimation}

It is well known result how greedy approximations are the best possible one for submodular, monotone maximization \cite{}. The result states that any approximation is at least $(1 - \frac{1}{e})$ close from the optimal result. This of course is a lower bound in the performance of our algorithm, an interesting question is if there is an upper bound for a particular set of interesting $\mu$.

Working in some theoretical results here


\section{Experiments}

Coming soon...





% Small number of stages experiments, think about experiments. 

% first formulates the trade-off between mean squared estimation error and regret via a minimax multi-objective optimization problem, then proposes a variation of the EXP3 algorithm (Auer et al. 2002)
% 2

% Intuitively, it is sensible that some degree of exploration must be imposed to produce inferential guarantees, as the precision of ATE inference essentially depends on the variance of the treatment arm which has the fewest number of observations.  por que?


% which takes draws from the estimated sub-optimal arms via a specified rate and shows that this adaptation satisfies this characterization of optimality. Intuitively, it is sensible that some degree of exploration must be imposed to produce inferential guarantees, as the precision of ATE inference essentially depends on the variance of the treatment arm which has the fewest number of observations.

% \cite{liang2023experimental} 


% Alternatively they talk about ($R_t(A_t) = R_t$):
% \begin{align*}
%     \E_{\pi^*}[R_t] - \E_{h_t}[R_t(A_t)]
% \end{align*}


% ============= Formalize the contextual Bandit setting using potential outcomes leanguage. =============

% In this context the value of a policy is the average treatment effect \Gap{Why is it not time dependant} 


% There is a potential outcome formulation for the OPE problem. Naturally this formulation is useful for studyng the \textit{sample} avergae treatment effect. Define
% \begin{align*}
%     \nu_t^* \equiv \E_{\pi}[R_t(G)|X^{t-1}_1] := &\int_{\mathcal{A}\times\mathcal{X}}\E[R_t(g)|G=g, X_t=x, X_{1}^{t-1}]\pi(g|x)p_{X_t}(x|X^{t-1}_1)dgdx\\
%                                                 &\E[\E_{G \sim \pi(\cdot | X_t)}[R_t(G)|X_t,X_1^{t-1}|X_1]|X_1^{t-1}]
% \end{align*}
% Where $R_t(G)$ is the potential outcome, i.e a different random variable that relates with the $R_t$ in the following way:
% \textbf{Consistency:} $A_t=a \rightarrow R_t(a)=R_t$ for every $a\in \mathcal{A}$ with positive $\pi-$ density.
% \textbf{Sequential ex-changeability:} $A_t \indep R_t(a) | X^t_{1} $
% \textbf{Positivity:} $\pi << h_t$.

% Then $$\nu^*_t = \nu_t$$

% Writing the definition of
% \begin{align}
%     \nu^*_t &:= \int_{\mathcal{A}\times\mathcal{X}}\E[R_t(g)|G=g, X_t=x, X_{1}^{t-1}]\pi(g|x)p_{X_t}(x|X^{t-1}_1)dgdx\\
%             &:= \int_{\mathcal{A}\times\mathcal{X}}\E[R_t(g)|A=g, G=g, X_t=x, X_{1}^{t-1}]\pi(g|x)p_{X_t}(x|X^{t-1}_1)dgdx\\
%             &:= \int_{\mathcal{A}\times\mathcal{X}}\E[R_t(g)|A=g, X_t=x, X_{1}^{t-1}]\pi(g|x)p_{X_t}(x|X^{t-1}_1)dgdx\\
%             &:= \int_{\mathcal{A}\times\mathcal{X}}\E[R_t|G=g, X_t=x, X_{1}^{t-1}]\pi(g|x)p_{X_t}(x|X^{t-1}_1)dgdx\\
%             & := \nu_t
% \end{align}

% Where in two it was used the sequential ex-changeability and in three the fact that \Gap{by definition, $R_t(G) \indep G|X_1^t$}. 


% What does this have to do with the aTE
% STOCASTIC INTERVENTIONS


% % \textbf{Example number two} Let $\mathcal{A} = \{-1, 1\}$, define $g^*( \cdot |X(t)) = (g_1( \cdot |X(t)) - g_0( \cdot |X(t))) $, where $g_1( \cdot |X(t))$ is the constant policy $1$ and $g_0( \cdot |X(t))$ is the constant policy $-1$. In this case, $g^*( \cdot |X(t))d\mu_{\mathcal{A}} = (\delta_{1} - \delta_{-1})$, and thus:
% \begin{align*}
%     \psi(Q_x, Q_Y) &= \int y Q_Y(dy|1,x)Q_x(dx) - \int y Q_Y(dy|-1,x)Q_x(dx)\\
%     \psi(Q_x, Q_Y) &= \int y(1) Q_Y(dy|1,x)Q_x(dx) - \int y(-1) Q_Y(dy|-1,x)Q_x(dx)\\
%     \psi(Q_x, Q_Y) &= \E[Y(1)] - \E[Y(-1)]
% \end{align*}



% The policies change over time in this setting $\{h_t\}_{t=1}^{\infty}$, we aim to balance context distributions between treatment arms (such as via Efron’s biased coin design [12]) or to adaptively find the treatment policy that yields the most efficient treatment effect estimators. In the literature for the OE this is not the case..., nor is it for the policy optimization probelm \Gap{Why?}


% How is this already a solved problem???? Understand RCT and bandits.


% IT is clear that both papers aim to produce confidence intervals for the OPE problem.

% ==================================================================================================================

% \section{Abstract}

% RCTs are expensive and require a significant amount of resources to set-up. Usually the deliverable after performing an RCT is an estimate of the ATE on top of which statistical inference can be performed. More formally, at the end of an RCT there should be statistical evidence of the realized intervention impact. However, in high-stakes settings in which  resources might be scarce (for example sending health officials to an area to increase vaccination rates), the cost of a wrong decision is very high. Thus, we aim to correctly identify at least a single good intervention. 
% Our proposal is to deliver a certificate for an intervention, meaning we will provide statistical evidence that at least one of the interventions is guaranteed to have a positive impact. To achieve this, we propose a warm-up stage to discard ineffective arms, thereby maximizing the power of our certificate in the second stage.


\section{Appendix}

\section{Top-k arm:} 
First some notation, let $k$ be the size of $B$. A \textit{top-k} strategy is such that $B$ is composed from the $k$ arms with the highest empirical means on the first stage. Lets begin by acknowledging the simple fact that $\E[\max_{i} X_i] \geq  \max_{i}\E[ X_i]$.
Another big change is that, as a consequence of the uniform allocation and that $|B|>1$, the initial Sub-Gaussian bound is transformed to $$\mu_i > \overline{Y}_i -\sqrt{\frac{2(b-a)^2}{|m/k|}log(\frac{2}{\delta})}$$.

Note how the size of $B$ is going to decrease the efficiency of the bound as a consequence of the term derived from the second stage:
\begin{align}
    \E[\E[\max_{i\in B} l_i| X]] &\geq \E[\max_{i\in B}\E[ \overline{Y}_i | X]] - C\left(\frac{log(\frac{1}{\delta})}{\sqrt{\frac{m}{|B|}}}\right)\\
    &\geq \E[\max_{i\in B}\mu_i] - C\left(\frac{log(\frac{1}{\delta})}{\sqrt{\frac{m}{|B|}}}\right)
\end{align}
Thus implying the fallowing bound on the regret:
\begin{align*}
    \E[\mu_{i^*} - max_{i \in B} l_i] \leq \E[\mu_{i^*} - \mu_J] + C\left(\frac{log(\frac{1}{\delta})}{\sqrt{\frac{m}{|B|}}}\right)
\end{align*}
Where $J = \argmax_{i \in B} \mu_i$. Note that now the second term does include the size of the set $B$ \textbf{however despite the similarity} the term $\E[\mu_{i^*} - \mu_J]$ has to be bounded by a term that is a function of the top-K algorithm, the easiest bound is just copy the procedure on \cite{bubeck2011pure}. With out loss of generality lets suppose that the arms are ordered by itts mean and that their mean reward is different (i.e $\mu_1 > \mu_2> ... > \mu_K$):
\begin{align*}
    \E[\mu_{i^*} - max_{i \in B} l_i] &\leq \E[\mu_{i^*} - max_{i\in B}\mu_i] + C\left(\frac{log(\frac{1}{\delta})}{\sqrt{\frac{m}{|B|}}}\right)\\
    \E[\mu_{i^*} - max_{i \in B} l_i] &\leq \sum_i \Delta_i P(1,..,i - 1  \notin B)  + C\left( \frac{log(\frac{1}{\delta})}{\sqrt{\frac{m}{|B|}}}\right)\\
     \E[\mu_{i^*} - max_{i \in B} l_i] &\leq \sum_i \Delta_i P(\overline{X}_i <\overline{X}_{(k)})  + C\left( \frac{log(\frac{1}{\delta})}{\sqrt{\frac{m}{|B|}}}\right)\\
    \E[\mu_{i^*} - max_{i \in B} l_i] &\leq \sum_{i}\Delta_i \prod_{l=1}^k\left( exp(-\frac{n}{K}\min_{(l)}\Delta_i^2) \right)    + C\left( \frac{log(\frac{1}{\delta})}{\sqrt{\frac{m}{|B|}}}\right)
\end{align*}
Where $\min_{(l)}$ means the $l$ smallest of the $\Delta_i$. The third line comes from the fact if its incurred in some regret is because, in particular, $i^* \notin B$. This is why the bound ends up depending in the fixed quantities of the top k smallest gaps; \textbf{there is not a clear way of how to deal with the order statistic derived from $\overline{X}_{(k)}$ in this case. Also this bound is too loose as it depends on $\min_i \Delta_i$ }

\textbf{Alternative approach} Remember that $k$ is he number of treatments chosen in the first stage and $K$ is the total number of treatments. Lets begin by defining $J = \argmax_{i \in B} \overline{Y}_i$, thus $J$ is the final selected treatment and is a random function of both $X$ and $Y$.
Let $e_n := P(J \neq i^*)$ be the probability of choosing the wrong best arm. Then,
\begin{align*}
       P(J \neq i^*) &\leq P(\overline{X}_{k} > \overline{X}_{i^*}) + P(\overline{Y}_{j} > \overline{Y}_{i^*})\\
      \leq & \left( exp(-\frac{n}{K}\min_{i}\Delta_i^2) \right)^{|B|} + P(\overline{Y}_{J} > \overline{Y}_{i^*} | \overline{X}_{k} \leq \overline{X}_{i^*})\\
      \leq & \left( exp(-\frac{n}{K}\min_{i}\Delta_i^2) \right)^{|B|} + exp\left(-\frac{m}{|B|}\min_{i}\Delta_i^2 \right) P(\overline{X}_{k} \leq \overline{X}_{i^*})\\
      &\leq \left( exp(-\frac{n}{K}\min_{i}\Delta_i^2) \right)^{|B|} + exp\left(-\frac{m}{|B|}\min_{i}\Delta_i^2\right)
\end{align*}

Where the first line comes from the two possible events related with $i^*$ being picked (or not) as part of the set $B$ for the first stage. The second line comes from applying the Hoeffding's bound same as it is done in \cite{bubeck2011pure}. As a consequence of the following inequality:
\begin{align*}
    \E[\mu_{i^*} - \mu_J] \leq e_n
\end{align*}
Then it can be concluded that:
\begin{align*}
     \E[\mu_{i^*} - max_{i \in B} l_i] &\leq \E[\mu_{i^*} - \mu_J] + C\left(\frac{log(\frac{1}{\delta})}{\sqrt{\frac{m}{|B|}}}\right)\\
     &\leq \left( exp(-\frac{n}{K}\min_{i}\Delta_i^2) \right)^{|B|} + exp\left(-\frac{m}{|B|}\min_{i}\Delta_i^2\right) + C\left(\frac{log(\frac{1}{\delta})}{\sqrt{\frac{m}{|B|}}}\right)
\end{align*}

\textbf{Now looking at this bound I feel uncomfortable, because it depends on the minimum gap. The former can be problematic because in scenarios where the minimum gap is small the bound is not very useful.}

Another idea is the following, let $\mu_{\rho}$ such that $\rho = \argmax_{i \in B} \overline{X}_i$ (Note that I could have use the less coarse definition $\rho = \argmax_{i \in B} \mu_i$, however is not true that a mistake can not happen if $\i^* \in B$). Then it must be true that:
\begin{align*}
    \E[\mu_{i^*} - \mu_B] + \E[\mu_{B} - \mu_J] \leq \sum_{i}\Delta_i P(\overline{X}{i^*} < \overline{X}_i)   + \sum_{i}\Delta_i P(\overline{Y}_{J} > \overline{Y}_{B}) 
\end{align*}
Here is straight forward to derive the bound by applying the bound from \cite{bubeck2011pure}:
\begin{align*}
    \E[\mu_{i^*} - \max_{i \in B}l_i] \leq \sum_{i}\Delta_i \left( exp(-\frac{n}{K}\Delta_i^2) \right) + \E[\mu_B - \mu_J]
\end{align*}
However, this last term is very difficult to deal with as it essentially compares $\max_{i} \overline{X}_i$ with $\max_{i \in B} \overline{Y}_i$.



\section{Threshold:} 
An analysis of the top-k arms can be difficult to perform, as there is not a clear path to analyze [...]. An interesting alternative will be to use a threshold to select the arms on the first stage. We proceed in the same way we did for the top-k approach:

\begin{align*}
    \E [\mu_{i^*} - l_i] &= \E [\mu_{i^*} - \overline{Y}_J] - \sqrt{\frac{log(1/\delta)}{m}}\E[\sqrt{|B|}]\\
                         &= \mu_{i^*} - \E[\max_{i \in B}\mu_i] - \sqrt{\frac{log(1/\delta)}{m}}\E[\sqrt{|B|}]\\
                         &= \mu_{i^*} - \E[\max_{i \in B}\mu_i] - \sqrt{\frac{log(1/\delta)}{m}}(\sum_i \sqrt{i} P(i = |B|) ) 
\end{align*}
With out loss of generality suppose the arms are sorted by their index and all means are different (i.e $\mu_1 > \mu_2 > ...> \mu_K$). Lets start by focusing on the term $\E[\mu_{1} - \max_{i \in B}\mu_i]$, the so called \textit{simple regret}. It is clear that in order to incur in some regret $\Delta_i$, then in particular $i$ must not belong to the set $B$:
\begin{align*}
     \E[\mu_{1} - \max_{i \in B}\mu_i] &\leq \sum_i \Delta_i P(1,..,i \notin B)
\end{align*}
Lets pick $\tau= \mu_\rho$ as the threshold, where $\rho$ is some number in $[K]$. Note that, as a result of Hoeffding's inequality :
\begin{align*}
    P(1,..,i-1 \notin B)  &= P(\overline{X}_{i} < \mu_\rho)\\
                                    &= P(\overline{X}_{i} - \mu_\rho -\Delta_{i\rho}) < - \Delta_{i\rho})\\
                                    &\leq exp(-\frac{n\Delta_{i\rho}^2}{2K})
\end{align*}
Where $\Delta_{i\rho} = \mu_i - \mu_{\rho}$, i.e, the relative gaps with respect to the threshold. These gaps unlike $\Delta_i$ can be negative. Hence, expanding our analysis even further:
\begin{align*}
    \E[\mu_{1} - \max_{i \ in B}\mu_i]  &\leq \sum_i \Delta_i P(1,..,i-1 \notin B)\\
                                        &\leq \sum_i \Delta_i \prod_{r=1}^i P(r\notin B)\\
                                        &\leq \sum_i \Delta_i exp(-\frac{n\sum_{r=1}^i\Delta_{r\rho}^2}{2K})
\end{align*}

Analyzing the size of the set $B$ is a bit more challenging, lets stick to $\mu_{\rho}$ as threshold. Let $A$ be the set of all tuples of size $i$ of elements in $[K]$. As consequence of the draw being independent it is clear that:
\begin{align*}
    P( |B| = i )  &\leq \sum_{\alpha \in A} exp\left(-\frac{n(\sum_{j \in \alpha} \Delta_{j\rho}^2)}{K}\right)\\
                  &\leq \sum_{\alpha \in A} exp\left(-\frac{ni(\max_{j \in \alpha}\Delta_{j\rho}^2)}{K}\right)\\
                  &\leq {K\choose i} exp\left(-\frac{n i(\max_{i}\Delta_{i\rho}^2)}{K}\right)
\end{align*}
Note how the bound can be made tighter by the means of combinatorial arguments. Instead of the last inequality, if the number of times a given element is the biggest element present in one of the tuples can be found, then that number can group a term that depends on $\max_{j \in \alpha}\Delta_{j\rho}^2)$.

Note that the argument, 
\begin{align*}
    P(\overline{X}_{i} < \mu_\rho) &= P(\overline{X}_{i} - \mu_\rho -\Delta_{i\rho}) < - \Delta_{i\rho})\\
                                   &\leq exp(-\frac{n\Delta_{i\rho}^2}{2K})
\end{align*}
Still hold if $\tau = \overline{X}_{\rho}$, thus our bounds still holds (this sounds wrong???).
\begin{align*}
    P(\overline{X}_{i} <  \overline{X}_{\rho}) &= P(\overline{X}_{i} -  \overline{X}_{\rho} -\Delta_{i\rho}) < - \Delta_{i\rho})\\
                                   &\leq exp(-\frac{n\Delta_{i\rho}^2}{2K})
\end{align*}

However this analysis leaves out the fact that everything is computed under the assumption that the order of the arms is known \Gap{Connect with Naveen's idea of using a prior}, will leave to two options:
\begin{itemize}
    \item Knowing $\rho$ before hand which would render the whole estimation superflous.
    \item Deal with the empirical distribution of the top-k, i.e : $  P(\overline{X}_{i} <  \overline{X}_{\rho})$ Which we know is hard.
\end{itemize}

Possible new directions to deal with this problem:

\begin{itemize}
    \item Use sample splitting to estimate the index $\rho$. In here, the first stage is split in to two samples. The first sample is used to estimate the order of the arms and the second to use such order to estimate the best size of $B$.

    \item Derive bounds by picking the set $B$ randomly. 
\end{itemize}

\section{Random B}
There must be at least one instance of a $B$ that is easy to analyze, the proposal is random. However even this entails some problems. Lets suppose that the size of $|B| = \rho$, i.e, $\rho$ arms are going to be randomly elected for the second stage. Then the bound becomes:
\begin{align*}
     \E[\mu_{i^*} - max_{i \in B} l_i] \leq \E[\mu_{i^*} - \mu_J] + C\left(\frac{log(\frac{1}{\delta})}{\sqrt{\frac{m}{|B|}}}\right)\\
     \E[\mu_{i^*} - max_{i \in B} l_i] \leq \E[\mu_{i^*} - \mu_J] + C\left(\frac{log(\frac{1}{\delta})\sqrt{\rho}}{\sqrt{m}}\right)\\
     \E[\mu_{i^*} - max_{i \in B} l_i] \leq \Pi_{i =1}^{\rho}\left( 1 - \frac{{K-i\choose \rho - i }}{{K\choose \rho}} \right) + C\left(\frac{log(\frac{1}{\delta})\sqrt{\rho}}{\sqrt{m}}\right)
\end{align*}
Which is hard to deal with, apart from the restrictions on the arms $\mu_{(i)}$ with $K - (\rho + 1) \leq i \leq K$ which simply can be the maximum arm picked in $B$.  Posible ideas to try next:

\begin{itemize}
    \item Try a grid just, 1 to s points to see what happens, is not data dependent. Union bound, on every point on the grid. empirical means of the arms?. Use the empirical mean among arms and use them to compare them. 
    \item error in the term of the estimate of your scond stage reward (yes, I think it should be the variance of the sample mean calculated on one half of the sample)

    \item Arent we falling in a circular argument by splitting the sampel in two to estimate things? Would it be better to go back to the top k approach?
    
\end{itemize}



\section{Uniform Threshold}

An even simpler idea is to use a grid of thresholds. Let discretize the interval $[0, 1]$ in $r$ pieces and lets fix $\tau$ as the threshold given by $\alpha/r$ where $\alpha \in [r]$. WALG suppose the means are ordered $\mu_{(1)}> \mu_{(2)}>...>\mu_{(k)}$. Let $\delta_{i\alpha} = \mu_{i} - \frac{\alpha}{r}$. The following the exact same argument as the one used in section 7:
\begin{align*}
    \E[\mu_{1} - \max_{i \ in B}\mu_i]  &\leq \sum_i \Delta_i P(1,..,i-1 \notin B)\\
                                        &\leq \sum_i \Delta_i \prod_{r=1}^i P(r\notin B)\\
                                        &\leq \sum_i \Delta_i exp(-\frac{n\sum_{r=1}^i\Delta_{i\alpha}^2}{2K})
\end{align*}

\newpage


==> sections/checklist.tex <==
\section*{Checklist}


 
 \begin{enumerate}
 \item For all models and algorithms presented, check if you include:
 \begin{enumerate}
   \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. [Yes]
   \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. [Yes]
   \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. [Yes]
 \end{enumerate}


 \item For any theoretical claim, check if you include:
 \begin{enumerate}
   \item Statements of the full set of assumptions of all theoretical results. [Yes]
   \item Complete proofs of all theoretical results. [Yes]
   \item Clear explanations of any assumptions. [Yes]     
 \end{enumerate}


 \item For all figures and tables that present empirical results, check if you include:
 \begin{enumerate}
   \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). [Yes]
   \item All the training details (e.g., data splits, hyperparameters, how they were chosen). [Yes/No/Not Applicable]
         \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). [Yes]
         \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). [Not Applicable]
 \end{enumerate}

 \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
 \begin{enumerate}
   \item Citations of the creator If your work uses existing assets. [Yes]
   \item The license information of the assets, if applicable. [Yes]
   \item New assets either in the supplemental material or as a URL, if applicable. [Yes]
   \item Information about consent from data providers/curators. [Not Applicable]
   \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. [Not Applicable]
 \end{enumerate}

 \item If you used crowdsourcing or conducted research with human subjects, check if you include:
 \begin{enumerate}
   \item The full text of instructions given to participants and screenshots. [Not Applicable]
   \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. [Not Applicable]
   \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. [Not Applicable]
 \end{enumerate}

 \end{enumerate}


==> sections/extensions.tex <==

\section{Extensions}

This work so far has been focused on bounding all possible choices of $\mu$. In particular, our bound  can be seen as an estimation of a min-max guarantee:
\begin{align*}
    \min_{\mu} \max_{\pi} f_\mu(\pi)
\end{align*}

Hence, without prior knowledge on the distribution, a bound dependant on the data is provided, thus guarantying a valid bound for all distributions $\mu$.

However, lets suppose for a moment that there is a prior on the distribution $\mu$. In this scenario our problem of interest gets reduced to:
\begin{align*}
    \min_{\rho \in U}\max_{\pi}f_{\mu}(\pi)
\end{align*}
Where $U$ bakes the prior knowledge on the distribution, reducing the problem to a subset of of distributions we are interested in. This presentation is usually refered in the literature as \textit{distributionally robust optimization}.

One special case of the previous setting is the so called \textit{stochastic regression} problem. On it, the distribution is fully known, thus reducing the problem to an stochastic optimization one.
\begin{align*}
    \max_{\pi}f_{\mu}(\pi)
\end{align*}

The dependency on $\mu$ can also be seen as a feature of this setting as it allows to encode prior information that might be available from the distribution. Such domain knowledge can be encoded in our problem as a Bayesian prior, thus making $\mu$ a random variable and transforming our objective into:

\begin{align*}
    \argmax_{\pi} \E_{\mu \sim P}[\E_{X \sim \mu}[f_{\mu}(\pi(X))]]
\end{align*}

 However, recall the fact that $f_{\mu}(\pi(X)) = \max_{\i \in B(X)} \mu_i - O(\sqrt{\frac{|B|}{m}})$, which leads to the question we faced in the min-max setting analyzed before; how can we approximate $ \max_{\i \in B(X)} \mu_i$? 

A possible solution will be to run a greedy search to craft the set $B$, as $\max$ is a submodular function. Then, the algorithm will compute via Montecarlo approximation a estimate of $E_{\mu \sim p(\mu|x)}[f_{\mu}(\pi(X))]$ and then greedily update the set $B$, thus creating an estimate for:
\begin{align*}
    \max_{|B| \leq k} \E_{\mu \sim p(\mu|x)}[f_{\mu}(\pi(X))]
\end{align*}

Which naturally will gave us an estimate of 
\begin{align*}
    \argmax_{\pi} \E_{\mu \sim p(\mu|x)}[f_{\mu}(\pi)]
\end{align*}

Note that 
\begin{align*}
    \E_{\mu \sim P}[\E_{X \sim \mu}[f_{\mu}(\pi(X))]] = \E_{X \sim \mu}[\E_{\mu \sim p(\mu|X)}[f_{\mu}(\pi(X))|X]] 
\end{align*}
Hence as $\pi$ is a function of $X$ the solution to the posterior will be the optimal.

\subsection{Upper bound on submodular estimation}

% It is well known result how greedy approximations are the best possible one for submodular, monotone maximization \cite{}. The result states that any approximation is at least $(1 - \frac{1}{e})$ close from the optimal result. This of course is a lower bound in the performance of our algorithm, an interesting question is if there is an upper bound for a particular set of interesting $\mu$.

Working in some theoretical results here


==> sections/random_b.tex <==


\section{Random B}
There must be at least one instance of a $B$ that is easy to analyze, the proposal is random. However even this entails some problems. Lets suppose that the size of $|B| = \rho$, i.e, $\rho$ arms are going to be randomly elected for the second stage. Then the bound becomes:
\begin{align*}
     \E[\mu_{i^*} - max_{i \in B} l_i] \leq \E[\mu_{i^*} - \mu_J] + C\left(\frac{log(\frac{1}{\delta})}{\sqrt{\frac{m}{|B|}}}\right)\\
     \E[\mu_{i^*} - max_{i \in B} l_i] \leq \E[\mu_{i^*} - \mu_J] + C\left(\frac{log(\frac{1}{\delta})\sqrt{\rho}}{\sqrt{m}}\right)\\
     \E[\mu_{i^*} - max_{i \in B} l_i] \leq \Pi_{i =1}^{\rho}\left( 1 - \frac{{K-i\choose \rho - i }}{{K\choose \rho}} \right) + C\left(\frac{log(\frac{1}{\delta})\sqrt{\rho}}{\sqrt{m}}\right)
\end{align*}
Which is hard to deal with, apart from the restrictions on the arms $\mu_{(i)}$ with $K - (\rho + 1) \leq i \leq K$ which simply can be the maximum arm picked in $B$.  Posible ideas to try next:

\begin{itemize}
    \item Try a grid just, 1 to s points to see what happens, is not data dependent. Union bound, on every point on the grid. empirical means of the arms?. Use the empirical mean among arms and use them to compare them. 
    \item error in the term of the estimate of your scond stage reward (yes, I think it should be the variance of the sample mean calculated on one half of the sample)

    \item Arent we falling in a circular argument by splitting the sampel in two to estimate things? Would it be better to go back to the top k approach?
    
\end{itemize}



==> sections/threshold.tex <==



\section{Threshold:} 
An analysis of the top-k arms can be difficult to perform, as there is not a clear path to analyze [...]. An interesting alternative will be to use a threshold to select the arms on the first stage. We proceed in the same way we did for the top-k approach:

\begin{align*}
    \E [\mu_{i^*} - l_i] &= \E [\mu_{i^*} - \overline{Y}_J] - \sqrt{\frac{log(1/\delta)}{m}}\E[\sqrt{|B|}]\\
                         &= \mu_{i^*} - \E[\max_{i \in B}\mu_i] - \sqrt{\frac{log(1/\delta)}{m}}\E[\sqrt{|B|}]\\
                         &= \mu_{i^*} - \E[\max_{i \in B}\mu_i] - \sqrt{\frac{log(1/\delta)}{m}}(\sum_i \sqrt{i} P(i = |B|) ) 
\end{align*}
With out loss of generality suppose the arms are sorted by their index and all means are different (i.e $\mu_1 > \mu_2 > ...> \mu_K$). Lets start by focusing on the term $\E[\mu_{1} - \max_{i \in B}\mu_i]$, the so called \textit{simple regret}. It is clear that in order to incur in some regret $\Delta_i$, then in particular $i$ must not belong to the set $B$:
\begin{align*}
     \E[\mu_{1} - \max_{i \in B}\mu_i] &\leq \sum_i \Delta_i P(1,..,i \notin B)
\end{align*}
Lets pick $\tau= \mu_\rho$ as the threshold, where $\rho$ is some number in $[K]$. Note that, as a result of Hoeffding's inequality :
\begin{align*}
    P(1,..,i-1 \notin B)  &= P(\overline{X}_{i} < \mu_\rho)\\
                                    &= P(\overline{X}_{i} - \mu_\rho -\Delta_{i\rho}) < - \Delta_{i\rho})\\
                                    &\leq exp(-\frac{n\Delta_{i\rho}^2}{2K})
\end{align*}
Where $\Delta_{i\rho} = \mu_i - \mu_{\rho}$, i.e, the relative gaps with respect to the threshold. These gaps unlike $\Delta_i$ can be negative. Hence, expanding our analysis even further:
\begin{align*}
    \E[\mu_{1} - \max_{i \ in B}\mu_i]  &\leq \sum_i \Delta_i P(1,..,i-1 \notin B)\\
                                        &\leq \sum_i \Delta_i \prod_{r=1}^i P(r\notin B)\\
                                        &\leq \sum_i \Delta_i exp(-\frac{n\sum_{r=1}^i\Delta_{r\rho}^2}{2K})
\end{align*}

Analyzing the size of the set $B$ is a bit more challenging, lets stick to $\mu_{\rho}$ as threshold. Let $A$ be the set of all tuples of size $i$ of elements in $[K]$. As consequence of the draw being independent it is clear that:
\begin{align*}
    P( |B| = i )  &\leq \sum_{\alpha \in A} exp\left(-\frac{n(\sum_{j \in \alpha} \Delta_{j\rho}^2)}{K}\right)\\
                  &\leq \sum_{\alpha \in A} exp\left(-\frac{ni(\max_{j \in \alpha}\Delta_{j\rho}^2)}{K}\right)\\
                  &\leq {K\choose i} exp\left(-\frac{n i(\max_{i}\Delta_{i\rho}^2)}{K}\right)
\end{align*}
Note how the bound can be made tighter by the means of combinatorial arguments. Instead of the last inequality, if the number of times a given element is the biggest element present in one of the tuples can be found, then that number can group a term that depends on $\max_{j \in \alpha}\Delta_{j\rho}^2)$.

Note that the argument, 
\begin{align*}
    P(\overline{X}_{i} < \mu_\rho) &= P(\overline{X}_{i} - \mu_\rho -\Delta_{i\rho}) < - \Delta_{i\rho})\\
                                   &\leq exp(-\frac{n\Delta_{i\rho}^2}{2K})
\end{align*}
Still hold if $\tau = \overline{X}_{\rho}$, thus our bounds still holds (this sounds wrong???).
\begin{align*}
    P(\overline{X}_{i} <  \overline{X}_{\rho}) &= P(\overline{X}_{i} -  \overline{X}_{\rho} -\Delta_{i\rho}) < - \Delta_{i\rho})\\
                                   &\leq exp(-\frac{n\Delta_{i\rho}^2}{2K})
\end{align*}

However this analysis leaves out the fact that everything is computed under the assumption that the order of the arms is known \Gap{Connect with Naveen's idea of using a prior}, will leave to two options:
\begin{itemize}
    \item Knowing $\rho$ before hand which would render the whole estimation superflous.
    \item Deal with the empirical distribution of the top-k, i.e : $  P(\overline{X}_{i} <  \overline{X}_{\rho})$ Which we know is hard.
\end{itemize}

Possible new directions to deal with this problem:

\begin{itemize}
    \item Use sample splitting to estimate the index $\rho$. In here, the first stage is split in to two samples. The first sample is used to estimate the order of the arms and the second to use such order to estimate the best size of $B$.

    \item Derive bounds by picking the set $B$ randomly. 
\end{itemize}

==> sections/top_k_arm.tex <==

\section{Top-k arm:} 
First some notation, let $k$ be the size of $B$. A \textit{top-k} strategy is such that $B$ is composed from the $k$ arms with the highest empirical means on the first stage. Lets begin by acknowledging the simple fact that $\E[\max_{i} X_i] \geq  \max_{i}\E[ X_i]$.
Another big change is that, as a consequence of the uniform allocation and that $|B|>1$, the initial Sub-Gaussian bound is transformed to $$\mu_i > \overline{Y}_i -\sqrt{\frac{2(b-a)^2}{|m/k|}log(\frac{2}{\delta})}$$.

Note how the size of $B$ is going to decrease the efficiency of the bound as a consequence of the term derived from the second stage:
\begin{align}
    \E[\E[\max_{i\in B} l_i| X]] &\geq \E[\max_{i\in B}\E[ \overline{Y}_i | X]] - C\left(\frac{log(\frac{1}{\delta})}{\sqrt{\frac{m}{|B|}}}\right)\\
    &\geq \E[\max_{i\in B}\mu_i] - C\left(\frac{log(\frac{1}{\delta})}{\sqrt{\frac{m}{|B|}}}\right)
\end{align}
Thus implying the fallowing bound on the regret:
\begin{align*}
    \E[\mu_{i^*} - max_{i \in B} l_i] \leq \E[\mu_{i^*} - \mu_J] + C\left(\frac{log(\frac{1}{\delta})}{\sqrt{\frac{m}{|B|}}}\right)
\end{align*}
Where $J = \argmax_{i \in B} \mu_i$. Note that now the second term does include the size of the set $B$ \textbf{however despite the similarity} the term $\E[\mu_{i^*} - \mu_J]$ has to be bounded by a term that is a function of the top-K algorithm, the easiest bound is just copy the procedure on \citep{bubeck2011pure}. With out loss of generality lets suppose that the arms are ordered by itts mean and that their mean reward is different (i.e $\mu_1 > \mu_2> ... > \mu_K$):
\begin{align*}
    \E[\mu_{i^*} - max_{i \in B} l_i] &\leq \E[\mu_{i^*} - max_{i\in B}\mu_i] + C\left(\frac{log(\frac{1}{\delta})}{\sqrt{\frac{m}{|B|}}}\right)\\
    \E[\mu_{i^*} - max_{i \in B} l_i] &\leq \sum_i \Delta_i P(1,..,i - 1  \notin B)  + C\left( \frac{log(\frac{1}{\delta})}{\sqrt{\frac{m}{|B|}}}\right)\\
     \E[\mu_{i^*} - max_{i \in B} l_i] &\leq \sum_i \Delta_i P(\overline{X}_i <\overline{X}_{(k)})  + C\left( \frac{log(\frac{1}{\delta})}{\sqrt{\frac{m}{|B|}}}\right)\\
    \E[\mu_{i^*} - max_{i \in B} l_i] &\leq \sum_{i}\Delta_i \prod_{l=1}^k\left( exp(-\frac{n}{K}\min_{(l)}\Delta_i^2) \right)    + C\left( \frac{log(\frac{1}{\delta})}{\sqrt{\frac{m}{|B|}}}\right)
\end{align*}
Where $\min_{(l)}$ means the $l$ smallest of the $\Delta_i$. The third line comes from the fact if its incurred in some regret is because, in particular, $i^* \notin B$. This is why the bound ends up depending in the fixed quantities of the top k smallest gaps; \textbf{there is not a clear way of how to deal with the order statistic derived from $\overline{X}_{(k)}$ in this case. Also this bound is too loose as it depends on $\min_i \Delta_i$ }

\textbf{Alternative approach} Remember that $k$ is he number of treatments chosen in the first stage and $K$ is the total number of treatments. Lets begin by defining $J = \argmax_{i \in B} \overline{Y}_i$, thus $J$ is the final selected treatment and is a random function of both $X$ and $Y$.
Let $e_n := P(J \neq i^*)$ be the probability of choosing the wrong best arm. Then,
\begin{align*}
       P(J \neq i^*) &\leq P(\overline{X}_{k} > \overline{X}_{i^*}) + P(\overline{Y}_{j} > \overline{Y}_{i^*})\\
      \leq & \left( exp(-\frac{n}{K}\min_{i}\Delta_i^2) \right)^{|B|} + P(\overline{Y}_{J} > \overline{Y}_{i^*} | \overline{X}_{k} \leq \overline{X}_{i^*})\\
      \leq & \left( exp(-\frac{n}{K}\min_{i}\Delta_i^2) \right)^{|B|} + exp\left(-\frac{m}{|B|}\min_{i}\Delta_i^2 \right) P(\overline{X}_{k} \leq \overline{X}_{i^*})\\
      &\leq \left( exp(-\frac{n}{K}\min_{i}\Delta_i^2) \right)^{|B|} + exp\left(-\frac{m}{|B|}\min_{i}\Delta_i^2\right)
\end{align*}

Where the first line comes from the two possible events related with $i^*$ being picked (or not) as part of the set $B$ for the first stage. The second line comes from applying the Hoeffding's bound same as it is done in \citep{bubeck2011pure}. As a consequence of the following inequality:
\begin{align*}
    \E[\mu_{i^*} - \mu_J] \leq e_n
\end{align*}
Then it can be concluded that:
\begin{align*}
     \E[\mu_{i^*} - max_{i \in B} l_i] &\leq \E[\mu_{i^*} - \mu_J] + C\left(\frac{log(\frac{1}{\delta})}{\sqrt{\frac{m}{|B|}}}\right)\\
     &\leq \left( exp(-\frac{n}{K}\min_{i}\Delta_i^2) \right)^{|B|} + exp\left(-\frac{m}{|B|}\min_{i}\Delta_i^2\right) + C\left(\frac{log(\frac{1}{\delta})}{\sqrt{\frac{m}{|B|}}}\right)
\end{align*}

\textbf{Now looking at this bound I feel uncomfortable, because it depends on the minimum gap. The former can be problematic because in scenarios where the minimum gap is small the bound is not very useful.}

Another idea is the following, let $\mu_{\rho}$ such that $\rho = \argmax_{i \in B} \overline{X}_i$ (Note that I could have use the less coarse definition $\rho = \argmax_{i \in B} \mu_i$, however is not true that a mistake can not happen if $\i^* \in B$). Then it must be true that:
\begin{align*}
    \E[\mu_{i^*} - \mu_B] + \E[\mu_{B} - \mu_J] \leq \sum_{i}\Delta_i P(\overline{X}{i^*} < \overline{X}_i)   + \sum_{i}\Delta_i P(\overline{Y}_{J} > \overline{Y}_{B}) 
\end{align*}
Here is straight forward to derive the bound by applying the bound from \citep{bubeck2011pure}:
\begin{align*}
    \E[\mu_{i^*} - \max_{i \in B}l_i] \leq \sum_{i}\Delta_i \left( exp(-\frac{n}{K}\Delta_i^2) \right) + \E[\mu_B - \mu_J]
\end{align*}
However, this last term is very difficult to deal with as it essentially compares $\max_{i} \overline{X}_i$ with $\max_{i \in B} \overline{Y}_i$.


==> sections/uniform_threshold.tex <==


\section{Uniform Threshold}

An even simpler idea is to use a grid of thresholds. Let discretize the interval $[0, 1]$ in $r$ pieces and lets fix $\tau$ as the threshold given by $\alpha/r$ where $\alpha \in [r]$. WALG suppose the means are ordered $\mu_{(1)}> \mu_{(2)}>...>\mu_{(k)}$. Let $\delta_{i\alpha} = \mu_{i} - \frac{\alpha}{r}$. The following the exact same argument as the one used in section 7:
\begin{align*}
    \E[\mu_{1} - \max_{i \ in B}\mu_i]  &\leq \sum_i \Delta_i P(1,..,i-1 \notin B)\\
                                        &\leq \sum_i \Delta_i \prod_{r=1}^i P(r\notin B)\\
                                        &\leq \sum_i \Delta_i exp(-\frac{n\sum_{r=1}^i\Delta_{i\alpha}^2}{2K})
\end{align*}

